SE(3) diffusion model with application to protein backbone generation

The design of novel protein structures remains a challenge in protein engineering for applications across biomedicine and chemistry. In this line of work, a diffusion model over rigid bodies in 3D (referred to as frames) has shown success in generating novel, functional protein backbones that have not been observed in nature. However, there exists no principled methodological framework for diffusion on SE(3), the space of orientation preserving rigid motions in R3, that operates on frames and confers the group invariance. We address these shortcomings by developing theoretical foundations of SE(3) invariant diffusion models on multiple frames followed by a novel framework, FrameDiff, for learning the SE(3) equivariant score over multiple frames. We apply FrameDiff on monomer backbone generation and find it can generate designable monomers up to 500 amino acids without relying on a pretrained protein structure prediction network that has been integral to previous methods. We find our samples are capable of generalizing beyond any known protein structure.

==> content/alternative_intro_text.tex <==
The ability to engineer novel proteins holds promise in developing
bio-therapeutics towards global health challenges such as SARS-COV-2
\citep{arunachalam2021adjuvanting} and cancer \citep{QUIJANORUBIO2020119}.
Unfortunately, efforts to engineer proteins require substantial domain
knowledge and laborious trial and error.  To this end, protein engineering has
greatly benefited from advancements in deep learning by automating knowledge
acquisition from data and improving efficiency in designing proteins
\citep{ding2022protein}.

Generating a novel protein satisfying
specified structural and functional properties is the task of \denovo{} protein
design \citep{huang2016coming}.
But generating novel proteins is technically challenging due to the coupling of structure
and sequence: atoms that comprise protein structure must adhere to physical and
chemical constraints.
In this paper we focus on protein backbone generation, including overall three-dimensional protein shape.
%The primary application is \emph{backbone generation} where the protein structure topology is determined.
A protein backbone consists of $\numres$ residues, each with
four heavy atoms rigidly connected via
covalent bonds, \bbatoms.
For generating backbones its important that they are ``designable" in the sense a sequence exists
that adopts the prescribed structure. 



However, current practice has outpaced theoretical foundations.
For example, \citet{watson2022rfdiffusion} demonstrated a diffusion model (RFdiffusion) to generate novel protein-binders with high, experimental-verified affinities,
but relied on a heuristic denoising loss and 
reported the inability to train without pretraining on protein structure prediction.
Our goal is to bridge this theory-practice gap.

The main technical challenge is to combine the expressive geometric deep learning methods that operate on protein structures with diffusion generative modeling.


As such, many successful computational methods for both protein structure prediction \citep{Jumper2021HighlyAP} and design \citep{watson2022rfdiffusion} represent backbone structures by an element of the Lie group $\SE(3)^N.$
Moreover, it is necessary to use $\SE(3)$ equivariant neural networks since biochemical function of proteins is conferred by the relative geometries of the atoms (and so are invariant to rigid transformations).
% Moreover, because the biochemical function of proteins is conferred by the relative geometries of the atoms that comprise them (and so are invariant to rigid transformations) typical neural networks on proteins operate with $\SE(3)$ equivariance.
%While \citet{debortoli2022Riemannian,huang2022Riemannian} have extended diffusion modeling to Riemannian manifolds, these works do not
% prescribe tractable training procedures or
%accommodate inclusion of geometric invariances.

%In this work, we develop the tools for diffusion on general Lie groups and their application to $\SE(3)^\numres;$ 


The present work contributes to both the theory and methodology of $\SE(3)$ diffusion models with applications to protein backbone generation.
On the theoretical side, we characterize
(a) the distribution of the Brownian motion on compact Lie groups (in particular $\SO(3)$) in a form amenable to denoising score matching training, and
(b) group invariance of Lie group diffusions, which for $\SE(3)^\numres$ we obtain through an $\SO(3)$ invariant \emph{centered} process.
We apply these contributions to develop \framediff{}, an $\SE(3)$ invariant diffusion model on $\SE(3)^\numres$ for protein backbones with roughly 4-fold fewer parameters than RFdiffusion and does not require pretraining.
We perform experiments on protein monomers and find that \framediff{}
can be trained to generate designable and diverse protein backbones up to length 500 that are occasionally novel compared to known proteins.
Compared to other methods, we report \emph{in-silico} designability success rates that are second only to RFdiffusion but far outperforming when RFdiffusion is trained from scratch.
% while far outperforming RFdiffusion trained from random initialization.
% While our focus is on protein backbone generation, we emphasize this is likely to be useful more broadly for example in Robotics applications on Lie groups.
Our contributions will enable further advancements in the $\SE(3)$ diffusion
methodology that underlies RFdiffusion and \framediff{} for proteins as well as
other domains such as robotics where $\SE(3)$ and other Lie groups are commonly used.

% We apply these contributions to develop \framediff{}, an $\SE(3)$ invariant diffusion model on $\SE(3)^\numres$.
% When trained on protein backbones, \framediff{}
% (a) generates up to 500 residue backbones that are diverse, designable, and novel compared known structures, and
% (b) with the inclusion of auxiliary losses which discourage physically implausible structures such as steric clashes in addition to a standard denoising score matching loss performs comparably to RFdiffusion, but with 5-fold fewer parameters and without requiring pre-training.
% While our focus is on protein backbone generation, we emphasize this is likely to be useful more broadly for example in Robotics applications on Lie groups.


==> content/introduction.tex <==
The ability to engineer novel proteins holds promise in developing
bio-therapeutics towards global health challenges such as SARS-COV-2
\citep{arunachalam2021adjuvanting} and cancer \citep{QUIJANORUBIO2020119}.
Unfortunately, efforts to engineer proteins require substantial domain
knowledge and laborious trial and error.  To this end, protein engineering has
greatly benefited from advancements in deep learning by automating knowledge
acquisition from data and improving efficiency in designing proteins
\citep{ding2022protein}.

Modeling proteins is technically challenging due to the coupling of structure
and sequence: atoms that comprise protein structure must adhere to physical and
chemical constraints while being ``designable" in the sense a sequence exists
that adopts the prescribed structure.  Generating a novel protein satisfying
specified structural and functional properties is the task of \denovo{} protein
design \citep{huang2016coming}.

The present work addresses the \emph{backbone generation} step of \denovo{}
protein design. A protein backbone consists of $\numres$ residues, each with
four heavy atoms\footnote{Nitrogen ($\texttt{N}$), two Carbons
  ($\texttt{C}_\alpha, \texttt{C}$), Oxygen ($\texttt{O}$).} connected via
covalent bonds, \bbatoms. In this work, we utilize an element of $\SE(3)$ called
a \emph{frame} (denoted as $T$) to parametrize each backbone atom of a residue.
Recovering absolute coordinates from frames has shown to result in highly
accurate predictions of X-ray crystallography protein structures
\citep{Jumper2021HighlyAP, baek2021accurate}.  It is also the most successful
parameterization for \denovo{} protein design \citep{watson2022rfdiffusion,
  wang2021deep, ingraham2022rfdiffusion, anishchenko2021novo}.


% Several approaches (and combination thereof) have
% explored the parameterization of the backbone structure.  Modeling Cartesian
% coordinates of each atom allows for unconstrained flexibility in atom placement,
% but comes at the cost of potentially violating bond constraints.  At the other
% extreme, using only torsion and dihedral angles will always satisfy bond
% constraints, but restricts movement of atoms to forward kinematics that becomes
% difficult to model for large proteins\footnote{This problem is known as the
%   \emph{lever arm effect}.} \citep{ingraham2018learning}.  A trade-off is to
% utilize a element of $\SE(3)$ called a \emph{frame} (denoted as $T$) to
% parametrize each backbone atom of a residue.  The frame construction has several
% advantages: (1) flexibility in atom placement by inferring $\calpha$
% coordinates; (2) modeling $\nitrogen, \carbon, \oxygen$ relative to $\calpha$
% with rotations that conserves all but one bond constraints.  Recovering absolute
% coordinates from frames has shown to result in highly accurate predictions of
% X-ray crystallography protein structures \citep{Jumper2021HighlyAP,
%   baek2021accurate}.  It is also the most successful parameterization for
% \denovo{} protein design \citep{watson2022rfdiffusion, wang2021deep,
%   ingraham2022rfdiffusion, anishchenko2021novo}.


% \valentin{you introduce the torsion angle but then we don't talk about it anymore.}
% \BLT{Jason and I have been going back and forth on this.  My preference would be to postpone discussion of the oxygen and torsion angle until a subsection of section 4.} \jason{I removed mention of the torsion angle here. Does that work? I think including mention of oxygen is still worthwhile.}
% \valentin{I am wondering if part of this discussion could be moved in Section 2 on Protein backbones}
% \jason{Brian and I went back and forth on this. I adopted his preference that having this in the introduction helps motivate the paper. It is a bit technical but hopefully not too much?}




When applied to backbone generation, diffusion models have significantly
advanced the ability to (a) generate novel structures beyond what has been
observed in nature and (b) control the generation towards desired functions.  In
particular, RFdiffusion \citep{watson2022rfdiffusion} achieved state-of-the-art
backbone generation by utilizing a pretrained protein folding network,
RosettaFold (RF) \citep{baek2021accurate}, within a diffusion model over
multiple $\SE(3)$ elements.  However, it was not shown whether the diffusion
framework in RFdiffusion is the theoretically correct approach for $\SE(3)$
diffusion.  Connecting the empirical success of RFdiffusion with theoretical
foundations is important for integrating methodological advances of diffusion
models in other domains.  Furthermore, RFdiffusion relies on RF, a pretrained 
60 million parameter neural network, that may burden usability in research
settings; \citet{watson2022rfdiffusion} reported the inability to train RFdiffusion without utilizing a pretrained protein folding network.

% \emile{Adding paragraph motivating probabilistic modelling on Lie groups and stating that we open the door to diffusion models on Lie groups}

Our contribution is twofold by (a) giving a rigorous treatment of $\SE(3)$
invariant diffusion models on multiple frames and (b) developing such a model,
called \framediff, over protein structures that does not require pretraining.
We perform experiments on protein monomer generation and find that \framediff{}
can be trained to generate designable and diverse protein backbones up to length
500 that can be unlike any protein backbone in the Protein Data Bank (PDB) \citep{berman2000protein}.  We compare our model's \emph{in silico}
designability success rate with RFdiffusion and Chroma
\citep{ingraham2022rfdiffusion} and find the success rate comparable to Chroma
while far outperforming RFdiffusion trained from random initialization.  Our
contributions will enable further advancements in the $\SE(3)$ diffusion
methodology that underlies RFdiffusion and \framediff{} for proteins as well as
other domains such as robotics where $\SE(3)$ and other Lie groups are commonly
used.



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:


==> content/software.tex <==

We used Python \citep{van1995python} for all programming, including PyTorch \citep{Paszke2019}, Hydra \citep{Yadan2019Hydra}, Numpy \citep{harris2020}, Scipy \citep{2020SciPy-NMeth}, Matplotlib \citep{Hunter2007}, Pandas \citep{mckinney2010data} and OpenFold \citep{ahdritz2022openfold}.

Code for $\SE(3)$ diffusion and FrameDiff: \url{https://github.com/jasonkyuyim/se3_diffusion}

==> content/sub_experiments/motif_scaffolding.tex <==
\TODO{Draft JY/BT}

\begin{table}[th]
\caption{Motif-scaffolding results.}
\label{sample-table}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lcccr}
\toprule
Data set & Naive & Flexible & Better? \\
\midrule
Breast    & 95.9$\pm$ 0.2& 96.7$\pm$ 0.2& $\surd$ \\
Cleveland & 83.3$\pm$ 0.6& 80.0$\pm$ 0.6& $\times$\\
Glass2    & 61.9$\pm$ 1.4& 83.8$\pm$ 0.7& $\surd$ \\
Credit    & 74.8$\pm$ 0.5& 78.3$\pm$ 0.6&         \\
Horse     & 73.3$\pm$ 0.9& 69.7$\pm$ 1.0& $\times$\\
Meta      & 67.1$\pm$ 0.6& 76.5$\pm$ 0.5& $\surd$ \\
Pima      & 75.1$\pm$ 0.6& 73.9$\pm$ 0.5&         \\
Vehicle   & 44.9$\pm$ 0.6& 61.5$\pm$ 0.4& $\surd$ \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table}

==> content/sub_methods/architecture.tex <==
\subsection{Score-network}
\label{sec:score_network}

% Neural network architecture for score.
The score network $\mathbf{s}_\theta$ aims to approximate each component of the Stein score $\nabla \log p_t(\bfT_t)$.
It is therefore parametrized as a map 
$\SE(3)^n \rightarrow \T\SE(3)^n$. 
\todo{@Valentin: introduce as section of tangent bundle?}
Let's denote by $T_{\text{global}} \in \SE(3)$ the global frame and by $T_i \in \SE(3)$ the local frame of the ith residue.
% following \cite{Jumper2021HighlyAP}, we parametrize the score network for each residue w.r.t.\ its local frame: ${\mathbf{s}}_\theta = \mathrm{T}^i \tilde{\mathbf{s}}_\theta$ with $\tilde{\mathbf{s}}_\theta$ an $\SE(3)$-invariant neural network.
% Hence ${\mathbf{s}}_\theta$ is trivially $\SE(3)$-equivariant since for all $\mathrm{T} \in \SE(3)$ we have that 
% $\mathrm{T} \cdot {\mathbf{s}}_\theta = {\mathbf{s}}_\theta \circ  \mathrm{T} = \mathrm{T}^i \tilde{\mathbf{s}}_\theta$
Following \cite{Jumper2021HighlyAP}, we parametrize  the score network in the \emph{local frame} of each residue with an $\SE(3)$-invariant self-attention architecture, yielding an $\SE(3)$-equivariant score in the \emph{global frame}.
\todo{last layer?}
\todo{how time $t$ is handled?}
In particular, we decompose it as $\mathbf{s}_\theta(t, T) = (T_i)_i \circ h_{\theta_K} \circ \dots \circ h_{\theta_1} \circ \text{emb}(t, T)$
where $\text{emb}$ and each self-attention layer $h_\theta$ are $\SE(3)$-invariant, thus yielding an $\SE(3)$-equivariant score $\mathbf{s}_\theta$.
% of $K$ layers $\left(\bm{v}^{k+1}_i\right)_{i\in(1,\cdots,N)} = \left( h_\theta \left(\bm{v}^{k}_i\right)\right)_{i\in(1,\cdots,N)}$ 
The layer update is defined as $s_i = h_\theta(\bm{s}) = (T_i)^{-1} \left( \sum_j a_{ij} T_j \mathbf{f}_\theta(s_j) \right)$,
where $s_i \in \R^m$ are the per-residue hidden features, $\mathbf{f}_\theta: \R^m \rightarrow \R^3$ the residue update (in the local frame) and $a_{ij} = a_{ij}(s_i, s_j, T_i, T_j) \in \R$ attention coefficients.
The attention module is based on a \emph{spatial} attention layer, Invariant Point Attention (IPA) \citep{Jumper2021HighlyAP}, which is biased towards spatially closed residue and a \emph{sequence} transformer attention layer that capture long range dependencies that may be far spatially.
%
Assuming that $\mathbf{f}_\theta$ and $a_{ij}$ are $\SE(3)$-invariant, we indeed have that $h_\theta$ is $\SE(3)$-invariant.
% since for any $\mathrm{T} \in \SE(3)$ we get
% $T \cdot h_\theta(\bm{v}_i) = (T T_i)^{-1} \left( \sum_j (T \cdot a_{ij}) T T_j  \mathbf{f}_\theta(T \bm{v}_j) \right) 
% = (T_i)^{-1} T^{-1} T \left( \sum_j a_{ij} T_j  \mathbf{f}_\theta(\bm{v}_j) \right)
% = h_\theta(\bm{v}_i)$.


==> content/sub_methods/previous_Riemannian_SBGM_recap.tex <==
We aim to construct and learn a diffusion model on the manifold
$\mathcal{M} \triangleq \SE(3)^N$.  As a \emph{group}
$\SE(3) \neq \SO(3) \times \R^3$ and can instead be described using a
semi-direct product $\SE(3) = \SO(3) \ltimes \R^3$. However, in
\Cref{sec:forw-diff-se3}, we show that choosing a specific metric on $\se(3)$,
$\SE(3)$ is a direct product between $\SO(3)$ and $\R^3$ from a \emph{metric}
point of view. Hence, a diffusion model on $\SE(3)$ can be rigorously
constructed as the product between a diffusion model on $\R^3$ and another one
$\SO(3)$. We discuss the implications of the choice of this metric on the
invariance/equivariance properties of the diffusion model in
\Cref{sec:inv_processes}.
% Although
% $\SE(3)= \SO(3) \ltimes \R^3 $ has a \emph{semi-direct group structure}, we show
% that from a diffusion model stance this is similar to constructing a diffusion
% on $\SO(3) \times \R^3$---see \cref{sec:metric-laplacian-se3}.
% % constructing a Brownian motion on $\SO(3) \times \R^3$ can be seen as a Brownian motion on $\SE(3)$ (as a group)---see \cref{sec:metric-laplacian-se3}.
% Since there is a priori no preferred position or pose for proteins, we would like to design a generative model that is invariant to the choice of frame.
% % Preserving the group structure is key when designing group invariant processes as shown in \cref{sec:inv_processes}.
% Hence preserving the group structure is key so as to design an $\SE(3)$ invariant processes as shown in \cref{sec:inv_processes}.
% % \cref{sec:invariant_process}.
% Combining these, in what follows we introduce $\SE(3)$-invariant continuous diffusion processes on $\SE(3)^N$.

\subsection{Forward noising process on manifolds}
%
In order to build a diffusion model on an (oriented) manifold
d$(\M, \mathfrak{g})$, one must first define a forward noising manifold-valued
process, transforming data into noise.  A broad class of processes can be
constructed as solutions of
SDEs, %, which involves a `noise term', usually a Brownian motion $(\bfB^\M_t)_{t \in \ccint{0,T}}$.
% The choice of metric $\mathfrak{g}$ is free, it enables doing calculus, e.g.\ constructing such SDEs but it also induces a Brownian motion, a volume form $\Vol$, an exponential map etc.
% A nice metric would be invariant w.r.t. the manifold isometries. % (transformations leaving the space unchanged).
which are usually driven by a Brownian motion $(\dt{\bfB_\M}{t})_{t \ge 0}$,
with distribution
$\mathbb{P}_t$ % $\mathbb{P}_t \triangleq \mathcal{L}(\dt{\bfB}{t})$
and density $p_t \triangleq \rmd \mathbb{P}_t / \rmd \Vol{\M}$.
%
% In what follows, we recall how to construct such a process following \cite{debortoli2022Riemannian}.
% Let $\M$ be a connected Riemannian manifold.
% We can define the process $(\bfX_t)_{t \in \ccint{0,T}}$ associated with the SDE
Following \citet{debortoli2022Riemannian}, we can construct a process $(\dt{\bfX}{t})_{t \in \ccint{0,T}}$ associated with the Langevin dynamics
\begin{equation}
  \label{eq:sde_manifold}
  \textstyle{
    \rmd \dt{\bfX}{t} = {- \tfrac{1}{2}\nabla U(\dt{\bfX}{t})} \rmd t + \rmd \dt{\bfB_\M}{t}, \quad \dt{\bfX}{0} \sim p_0 ,
    }
\end{equation}
which admits the invariant density $\piinv(x) \propto \rme^{-U(x)}$, under some
regularity assumption on $U$.
% For such a forward process the backward diffusion is given by the following proposition.
The backward diffusion of this forward process is given by the following proposition.
%
\begin{proposition}[\citet{debortoli2022Riemannian}]
  Under mild assumption on $p_0$, the time-reversal process
  $(\dt{\bfY}{t})_{t \in \ccint{0,T}} = (\dt{\bfX}{T-t})_{t \in \ccint{0,T}}$ is
  solution of the following SDE
  \begin{equation*}
    \label{eq:time_reversal_manifold}
    \textstyle{
      \rmd \dt{\bfY}{t} = \cbr{\tfrac{1}{2} \nabla U(\dt{\bfY}{t})+ \nabla \log p_{T-t}(\dt{\bfY}{t})} \rmd t + \rmd \dt{\bfB_\M}{t}.
      }
  \end{equation*}
\end{proposition}
%
The quantity $\nabla \log p_t$ is called the Stein score and is unavailable in
practice. It is approximated with a score network
$\mathbf{s}_\theta(t,\cdot) \approx \nabla \log p_{t}$ which is trained by
minimising a denoising score matching ($\mathrm{dsm}$) loss
  \begin{equation}
    \label{eq:desnoing_sm}
    \textstyle{
    \mathcal{L}(\mathbf{s}_\theta) = \E [ \norm{ \nabla \log p_{t|0}(\dt{\bfX}{t}|\dt{\bfX}{0}) -
      \mathbf{s}_\theta(t, \dt{\bfX}{t}) }^2],
  }
    % \textstyle{
    % \mathcal{L}_{\rm{dsm}}(\mathbf{s}_\theta) = \E [ \lambda_t \norm{ \nabla_{\dt{\bfX}{t}} \log p_{t|0}(\dt{\bfX}{t}|\dt{\bfX}{0}) -
    %   \mathbf{s}_\theta(t, \dt{\bfX}{t}) }^2]
    % }  
  \end{equation}
  where the expectation is defined over
  $(\dt{\bfX}{0}, \dt{\bfX}{t})$\footnote{In practice, we consider
    weighted versions of the loss.}.  Next, we describe the key
  ingredients to apply this framework in $\rset^3$ and $\SO(3)$ in order to
  derive a principled diffusion model on $\SE(3)$.

